On Fast Decoding of High Dimensional Signals from One-Bit Measurements

In the problem of one-bit compressed sensing, the goal is to find a $\delta$-close estimation of a $k$-sparse vector $x \in \mathbb{R}^n$ given the signs of the entries of $y = \Phi x$, where $\Phi$ is called the measurement matrix. For the one-bit compressed sensing problem, previous work \cite{Plan-robust,support} achieved $\Theta (\delta^{-2} k \log(n/k))$ and $\tilde{ \Oh} ( \frac{1}{ \delta } k \log (n/k))$ measurements, respectively, but the decoding time was $\Omega ( n k \log (n / k ))$. \ In this paper, using tools and techniques developed in the context of two-stage group testing and streaming algorithms, we contribute towards the direction of very fast decoding time. We give a variety of schemes for the different versions of one-bit compressed sensing, such as the for-each and for-all version, support recovery; all these have $poly(k, \log n)$ decoding time, which is an exponential improvement over previous work, in terms of the dependence of $n$.

==> bibio <==
@article{cormode2005improved,
  title={An improved data stream summary: the count-min sketch and its applications},
  author={Cormode, Graham and Muthukrishnan, S},
  journal={Journal of Algorithms},
  volume={55},
  number={1},
  pages={58--75},
  year={2005},
  publisher={Elsevier}
}

@incollection{HPA,
year={2011},
isbn={978-3-642-22005-0},
booktitle={Automata, Languages and Programming},
volume={6755},
series={Lecture Notes in Computer Science},
editor={Aceto, Luca and Henzinger, Monika and Sgall, Jiří},
doi={10.1007/978-3-642-22006-7_47},
title={Efficiently Decodable Error-Correcting List Disjunct Matrices and Applications},
url={http://dx.doi.org/10.1007/978-3-642-22006-7_47},
publisher={Springer Berlin Heidelberg},
author={Ngo, HungQ. and	 Porat, Ely and Rudra, Atri},
pages={557-568},
language={English}
}


@inproceedings{Porat2,
  author    = {Anna C. Gilbert and
               Yi Li and
               
 Ely Porat and
               Martin J. Strauss},
  title     = {For-All Sparse Recovery in Near-Optimal Time},
  booktitle = {Automata, Languages, and Programming - 41st International Colloquium,
               {ICALP} 2014, Copenhagen, Denmark, July 8-11, 2014, Proceedings, Part
               {I}},
  pages     = {538--550},
  year      = {2014},
  crossref  = {DBLP:conf/icalp/2014-1},
  url       = {http://dx.doi.org/10.1007/978-3-662-43948-7_45},
  doi       = {10.1007/978-3-662-43948-7_45},
  timestamp = {Fri, 13 Jun 2014 13:51:35 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icalp/GilbertLPS14},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Tao, 
author={Candes, E.J. and Tao, T.}, 
journal={Information Theory, IEEE Transactions on}, 
title={Near-Optimal Signal Recovery From Random Projections: Universal Encoding Strategies?}, 
year={2006}, 
volume={52}, 
number={12}, 
pages={5406-5425}, 
keywords={encoding;linear programming;signal reconstruction;N-dimensional Gaussian vector;linear measurement;linear program;random projection;signal reconstruction;signal recovery;universal encoding strategy;Concrete;Digital images;Encoding;Geometry;Image coding;Image reconstruction;Linear programming;Mathematics;Measurement standards;Vectors;Concentration of measure;convex optimization;duality in optimization;linear programming;random matrices;random projections;signal recovery;singular values of random matrices;sparsity;trigonometric expansions;uncertainty principle}, 
doi={10.1109/TIT.2006.885507}, 
ISSN={0018-9448}, 
month={Dec},}

@article{chen2001atomic,
  title={Atomic decomposition by basis pursuit},
  author={Chen, Scott Shaobing and Donoho, David L and Saunders, Michael A},
  journal={SIAM review},
  volume={43},
  number={1},
  pages={129--159},
  year={2001},
  publisher={SIAM}
}


@article{plan2013one,
  title={One-Bit Compressed Sensing by Linear Programming},
  author={Plan, Yaniv and Vershynin, Roman},
  journal={Communications on Pure and Applied Mathematics},
  volume={66},
  number={8},
  pages={1275--1297},
  year={2013},
  publisher={Wiley Online Library}
}


@article{Plan-robust,
  title={Robust 1-bit compressed sensing and sparse logistic regression: A convex programming approach},
  author={Plan, Yaniv and Vershynin, Roman},
  journal={Information Theory, IEEE Transactions on},
  volume={59},
  number={1},
  pages={482--494},
  year={2013},
  publisher={IEEE}
}


@inproceedings{CandesTao,
  title={Error correction via linear programming},
  author={Candes, Emmanuel and Rudelson, Mark and Tao, Terence and Vershynin, Roman},
  booktitle={Foundations of Computer Science, 2005. FOCS 2005. 46th Annual IEEE Symposium on},
  pages={668--681},
  year={2005},
  organization={IEEE}
}

@proceedings{dam,
  editor    = {Rudolf Ahlswede and
               Lars B{\"{a}}umer and
               Ning Cai and
               Harout K. Aydinian and
               Vladimir Blinovsky and
               Christian Deppe and
               Haik Mashurian},
  title     = {General Theory of Information Transfer and Combinatorics},
  series    = {Lecture Notes in Computer Science},
  volume    = {4123},
  publisher = {Springer},
  year      = {2006},
  isbn      = {3-540-46244-9},
  timestamp = {Thu, 21 Dec 2006 12:43:59 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/gtitc/2006},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{Baraniuk,
  author    = {Laurent Jacques and
               Jason N. Laska and
               Petros T. Boufounos and
               Richard G. Baraniuk},
  title     = {Robust 1-Bit Compressive Sensing via Binary Stable Embeddings of Sparse
               Vectors},
  journal   = {{IEEE} Transactions on Information Theory},
  volume    = {59},
  number    = {4},
  pages     = {2082--2102},
  year      = {2013},
  url       = {http://dx.doi.org/10.1109/TIT.2012.2234823},
  doi       = {10.1109/TIT.2012.2234823},
  timestamp = {Tue, 09 Apr 2013 19:57:48 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/tit/JacquesLBB13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{bio,
  author    = {Raghunandan M. Kainkaryam and
               Angela Bruex and
               Anna C. Gilbert and
               John Schiefelbein and
               Peter J. Woolf},
  title     = {poolMC: Smart pooling of mRNA samples in microarray experiments},
  journal   = {{BMC} Bioinformatics},
  volume    = {11},
  pages     = {299},
  year      = {2010},
  url       = {http://dx.doi.org/10.1186/1471-2105-11-299},
  doi       = {10.1186/1471-2105-11-299},
  timestamp = {Thu, 01 Jul 2010 14:42:12 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/bmcbi/KainkaryamBGSW10},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{mut,
  author    = {S. Muthukrishnan},
  title     = {Data Streams: Algorithms and Applications},
  journal   = {Foundations and Trends in Theoretical Computer Science},
  volume    = {1},
  number    = {2},
  year      = {2005},
  url       = {http://dx.doi.org/10.1561/0400000002},
  doi       = {10.1561/0400000002},
  timestamp = {Tue, 20 May 2008 12:36:33 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/fttcs/Muthukrishnan05},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{Donoho,
  author    = {David L. Donoho},
  title     = {Compressed sensing},
  journal   = {{IEEE} Transactions on Information Theory},
  volume    = {52},
  number    = {4},
  pages     = {1289--1306},
  year      = {2006},
  url       = {http://dx.doi.org/10.1109/TIT.2006.871582},
  doi       = {10.1109/TIT.2006.871582},
  timestamp = {Mon, 31 Oct 2011 17:05:18 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/tit/Donoho06},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@inproceedings{first,
  author    = {Petros Boufounos and
               Richard G. Baraniuk},
  title     = {1-Bit compressive sensing},
  booktitle = {42nd Annual Conference on Information Sciences and Systems, CISS
               2008, Princeton, NJ, USA, 19-21 March 2008},
  pages     = {16--21},
  year      = {2008},
  crossref  = {DBLP:conf/ciss/2008},
  url       = {http://dx.doi.org/10.1109/CISS.2008.4558487},
  doi       = {10.1109/CISS.2008.4558487},
  timestamp = {Wed, 15 Oct 2014 17:04:27 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/ciss/BoufounosB08},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@article{pooling,
  author    = {Fei{-}Huang Chang and
               Huilan Chang and
               Frank K. Hwang},
  title     = {Pooling designs for clone library screening in the inhibitor complex
               model},
  journal   = {J. Comb. Optim.},
  volume    = {22},
  number    = {2},
  pages     = {145--152},
  year      = {2011},
  url       = {http://dx.doi.org/10.1007/s10878-009-9279-9},
  doi       = {10.1007/s10878-009-9279-9},
  timestamp = {Thu, 27 Feb 2014 07:41:03 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/jco/ChangCH11},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}



@article{angle,
  author    = {Hong{-}Bin Chen and
               Frank K. Hwang},
  title     = {A survey on nonadaptive group testing algorithms through the angle
               of decoding},
  journal   = {J. Comb. Optim.},
  volume    = {15},
  number    = {1},
  pages     = {49--59},
  year      = {2008},
  url       = {http://dx.doi.org/10.1007/s10878-007-9083-3},
  doi       = {10.1007/s10878-007-9083-3},
  timestamp = {Wed, 12 Mar 2008 12:47:07 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/jco/ChenH08},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{dorfman1943,
author = {Dorfman, Robert},
doi = {10.1214/aoms/1177731363},
fjournal = {The Annals of Mathematical Statistics},
journal = {Ann. Math. Statist.},
month = {12},
number = {4},
pages = {436--440},
publisher = {The Institute of Mathematical Statistics},
title = {The Detection of Defective Members of Large Populations},
url = {http://dx.doi.org/10.1214/aoms/1177731363},
volume = {14},
year = {1943}
}



@inproceedings{support,
  title={One-bit compressed sensing: Provable support and vector recovery},
  author={Gopi, Sivakant and Netrapalli, Praneeth and Jain, Prateek and Nori, Aditya},
  booktitle={Proceedings of the 30th international conference on machine learning (ICML-13)},
  pages={154--162},
  year={2013}

}


@article{phase29,
author = {Gonsalves, Robert A.},
title = {Phase Retrieval And Diversity In Adaptive Optics},
journal = {Optical Engineering},
volume = {21},
number = {5},
pages = {215829-215829-},
year = {1982},
isbn = {0091-3286},
doi = {10.1117/12.7972989},
URL = { http://dx.doi.org/10.1117/12.7972989},
eprint = {}
}

@article{phase30,
  title={Optical wavefront reconstruction: Theory and numerical methods},
  author={Luke, D Russell and Burke, James V and Lyon, Richard G},
  journal={SIAM review},
  volume={44},
  number={2},
  pages={169--224},
  year={2002},
  publisher={Society for Industrial and Applied Mathematics}
}

@article{phase31, 
author = {Anthony Cheetham and Nick Cvetojevic and Barnaby Norris and Anand Sivaramakrishnan and Peter Tuthill}, 
journal = {Opt. Express}, 
keywords = {Interferometry; Space instrumentation ; Active or adaptive optics},
number = {11}, 
pages = {12924--12934}, 
publisher = {OSA},
title = {Fizeau interferometric cophasing of segmented mirrors: experimental validation}, 
volume = {22}, 
month = {Jun},
year = {2014},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-22-11-12924},
doi = {10.1364/OE.22.012924},
}


@article{phase34, 
author = {Adolf W. Lohmann and Gerd Weigelt and Bernhard Wirnitzer}, 
journal = {Appl. Opt.}, 
keywords = {},
number = {24}, 
pages = {4028--4037}, 
publisher = {OSA},
title = {Speckle masking in astronomy: triple correlation theory and applications}, 
volume = {22}, 
month = {Dec},
year = {1983},
url = {http://ao.osa.org/abstract.cfm?URI=ao-22-24-4028},
doi = {10.1364/AO.22.004028},
abstract = {Due to the turbulent atmosphere the resolution of conventional astrophotography is limited to $\sim$1 sec of arc. However, the speckle-masking method can yield diffraction-limited resolution, i.e., 0.03 sec of arc with a 3.6-m telescope. Speckle masking yields true images of general astronomical objects. No point source is required in the isoplanatic field of the object. We present the theory of speckle masking; it makes use of triple correlations and their Fourier counterparts, the bispectra. We show algorithms for the recovery of the object from genuine astronomical bispectra data.},
}


@book{ phase35,
editor = "François Roddier",
title = {Adaptive Optics in Astronomy}, 
publisher = {Cambridge University Press}, 
year = {1999},
isbn = {9780511525179}, 
note = {Cambridge Books Online}, 
url = {http://dx.doi.org/10.1017/CBO9780511525179}
}

@article{phase38,
  title={Phaselift: Exact and stable signal recovery from magnitude measurements via convex programming},
  author={Candes, Emmanuel J and Strohmer, Thomas and Voroninski, Vladislav},
  journal={Communications on Pure and Applied Mathematics},
  volume={66},
  number={8},
  pages={1241--1274},
  year={2013},
  publisher={Wiley Online Library}
}

@inproceedings{phase40,
  title={Efficient compressive phase retrieval with constrained sensing vectors},
  author={Bahmani, Sohail and Romberg, Justin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={523--531},
  year={2015}
}

@inproceedings{phase41,
  title={Compressive phase retrieval},
  author={Moravec, Matthew L and Romberg, Justin K and Baraniuk, Richard G},
  booktitle={Optical Engineering+ Applications},
  pages={670120--670120},
  year={2007},
  organization={International Society for Optics and Photonics}
}


@article{phase43,
  author = {A. S. Bandeira and J. Cahil and D. G. Mixon and A. A. Nelson},
  title = {Saving phase: Injectivity and stability for phase retrieval},
  journal = {Applied and Computational Harmonic Analysis (ACHA)},
    volume = {37},
    pages = {106-125},
  year = {2014}
}

@article{phase44,
  title={Sparsity constrained nonlinear optimization: Optimality conditions and algorithms},
  author={Beck, Amir and Eldar, Yonina C},
  journal={SIAM Journal on Optimization},
  volume={23},
  number={3},
  pages={1480--1509},
  year={2013},
  publisher={SIAM}
}





@ARTICLE{phase32,
   author = {{Labeyrie}, A.},
    title = {Attainment of Diffraction Limited Resolution in Large Telescopes by Fourier Analysing Speckle Patterns in Star Images},
  journal = {Astronomy and Astrophysics},
     year = {1970},
    month = {may},
   volume = {6},
    pages = {85},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{phase33,
  title={Phase retrieval and image reconstruction for astronomy},
  author={Fienup, C and Dainty, J},
  journal={Image Recovery: Theory and Application},
  pages={231--275},
  year={1987},
  publisher={San Diego, CA, USA: Academic}
}


@BOOK{phase36,
   author = {{Roddier}, F.},
    title = "{Adaptive Optics in Astronomy}",
booktitle = {Adaptive Optics in Astronomy, Edited by Fran{\c c}ois Roddier, pp.~419.~ISBN 0521612144.~Cambridge, UK: Cambridge University Press, November 2004.},
     year = 2004,
    month = nov,
    pages = {419},
   adsurl = {http://adsabs.harvard.edu/abs/2004aoa..book.....R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@article{phase45,
title= { Sparsity-based single-shot subwavelength coherent diffractive imaging},
author = { Szameit, A., Shechtman, Y., Osherovich, E., Bullkich, E., Sidorenko, P., Dana, H., Steiner, S., Kley, E. B., Gazit, S., Cohen-Hyams, T., Shoham, S., Zibulevsky, M., Yavneh, I., Eldar, Y. C., Cohen, O., Segev, M.}
journal = {Nature},
publisher ={Nature Publishing Group},
pages={ 1476-1122}
 
}


@ARTICLE{jacques, 
author={Jacques, L. and Laska, J.N. and Boufounos, P.T. and Baraniuk, R.G.}, 
journal={Information Theory, IEEE Transactions on}, 
title={Robust 1-Bit Compressive Sensing via Binary Stable Embeddings of Sparse Vectors}, 
year={2013}, 
volume={59}, 
number={4}, 
pages={2082-2102}, 
keywords={Gaussian processes;analogue-digital conversion;probability;signal reconstruction;signal sampling;vectors;ADC;CS framework;analog-to-digital converters;binary ε-stable embedding property;binary stable embedding;ideal reconstruction;measurement robust mapping;noiseless measurements;optimal error decay;overwhelming probability;random Gaussian matrices;robust compressive sensing;sampling rate;signal reconstruction;sparse vector;word length 1 bit;Decoding;Distortion measurement;Measurement uncertainty;Noise measurement;Quantization;Robustness;Vectors;1-bit compressed sensing;approximation error;compressed sensing;consistent reconstruction;dimensionality reduction;iterative reconstruction;quantization;reconstruction algorithms;signal reconstruction;sparsity}, 
doi={10.1109/TIT.2012.2234823}, 
ISSN={0018-9448}, 
month={April},}

@ARTICLE{laska,
author={Laska, J.N. and Zaiwen Wen and Wotao Yin and Baraniuk, R.G.}, 
journal={Signal Processing, IEEE Transactions on}, 
title={Trust, But Verify: Fast and Accurate Signal Recovery From 1-Bit Compressive Measurements}, 
year={2011}, 
volume={59}, 
number={11}, 
pages={5289-5301}, 
keywords={concave programming;signal detection;signal processing;Shannon-Nyquist rate;analog-to-digital converter;compressive sensing;nonconvex optimization;restricted-step shrinkage;signal acquisition;signal recovery;word length 1 bit;Atmospheric measurements;Compressed sensing;Convergence;Hardware;Optimization;Particle measurements;Quantization;1-Bit compressive sensing;consistent reconstruction;quantization;trust-region algorithms}, 
doi={10.1109/TSP.2011.2162324}, 
ISSN={1053-587X}, 
month={Nov},}
}


@inproceedings{gupta,
  title={Sample complexity for 1-bit compressed sensing and sparse classification.},
  author={Gupta, Ankit and Nowak, Robert D and Recht, Benjamin},
  booktitle={ISIT},
  pages={1553--1557},
  year={2010}
}


@article{fase43, 
author = {Yoav Shechtman and Yonina C. Eldar and Alexander Szameit and Mordechai Segev}, 
journal = {Opt. Express}, 
keywords = {Image reconstruction techniques; Partial coherence in imaging; Microscopy},
number = {16}, 
pages = {14807--14822}, 
publisher = {OSA},
title = {Sparsity based sub-wavelength imaging with partially incoherent light via quadratic compressed sensing}, 
volume = {19}, 
month = {Aug},
year = {2011},
url = {http://www.opticsexpress.org/abstract.cfm?URI=oe-19-16-14807},
doi = {10.1364/OE.19.014807},
abstract = {We demonstrate that sub-wavelength optical images borne on partially-spatially-incoherent light can be recovered, from their far-field or from the blurred image, given the prior knowledge that the image is sparse, and only that. The reconstruction method relies on the recently demonstrated sparsity-based sub-wavelength imaging. However, for partially-spatially-incoherent light, the relation between the measurements and the image is quadratic, yielding non-convex measurement equations that do not conform to previously used techniques. Consequently, we demonstrate new algorithmic methodology, referred to as quadratic compressed sensing, which can be applied to a range of other problems involving information recovery from partial correlation measurements, including when the correlation function has local dependencies. Specifically for microscopy, this method can be readily extended to white light microscopes with the additional knowledge of the light source spectrum.},
}


@INPROCEEDINGS{fase23, 
author={Jaganathan, K. and Oymak, S. and Hassibi, B.}, 
booktitle={Information Theory Proceedings (ISIT), 2012 IEEE International Symposium on}, 
title={Recovery of sparse 1-D signals from the magnitudes of their Fourier transform}, 
year={2012}, 
pages={1473-1477}, 
keywords={Fourier transforms;combinatorial mathematics;convex programming;probability;signal reconstruction;Fourier transform;combinatorial analysis;convex optimization based framework;noniterative recovery algorithms;numerical simulations;one-dimensional signals;probability;sparse 1D signal recovery;Algorithm design and analysis;Convex functions;Correlation;Fourier transforms;Manifolds;Optimized production technology;Random variables;Autocorrelation;Convex Optimization;Phase Retrieval;Sparse Spectral Factorization}, 
doi={10.1109/ISIT.2012.6283508}, 
ISSN={2157-8095}, 
month={July},}


@article{fase2,
  author    = {Amir Beck and
               Yonina C. Eldar},
  title     = {Sparsity Constrained Nonlinear Optimization: Optimality Conditions
               and Algorithms},
  journal   = {CoRR},
  volume    = {abs/1203.4580},
  year      = {2012},
  url       = {http://arxiv.org/abs/1203.4580},
  timestamp = {Wed, 10 Oct 2012 21:28:49 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/abs-1203-4580},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{fase42, 
author={Shechtman, Y. and Beck, A. and Eldar, Y.C.}, 
booktitle={Electrical Electronics Engineers in Israel (IEEEI), 2012 IEEE 27th Convention of}, 
title={Efficient phase retrieval of sparse signals}, 
year={2012}, 
pages={1-5}, 
keywords={Fourier transforms;search problems;signal processing;1D phase retrieval;1D signal recovery;Fourier phase information;Fourier transform magnitude measurement;fast local search method;matrix lifting;nonzero element;one dimensional phase retrieval;sparse recovering;sparse signal retrieval;Correlation;Discrete Fourier transforms;Indexes;Linear programming;Runtime;Sparse matrices;Vectors}, 
doi={10.1109/EEEI.2012.6376967}, 
month={Nov},}


@article{faseyonina,
  title={Phase retrieval: Stability and recovery guarantees},
  author={Eldar, Yonina C and Mendelson, Shahar},
  journal={Applied and Computational Harmonic Analysis},
  volume={36},
  number={3},
  pages={473--494},
  year={2014},
  publisher={Elsevier}
}


@inproceedings{foreach1,
  title={Fast compressive phase retrieval from Fourier measurements},
  author={Yapar, Cagkan and Pohl, Volker and Boche, Holger},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2015 IEEE International Conference on},
  pages={3267--3271},
  year={2015},
  organization={IEEE}
}

@article{foreach2,
author = {Sheng Cai and Bakshi, M. and Jaggi, S. and Minghua Chen},
title= { SUPER: Sparse signals with unknown phases efficiently recovered},
journal={ Information Theory (ISIT), IEEE International Symposium} ,
year = {2014},
volume ={ vol., no., pp.2007-2011},
url= {doi: 10.1109/ISIT.2014.6875185},
}


@article{tarokh22,
  title={Sparse signal recovery from quadratic measurements via convex programming},
  author={Li, Xiaodong and Voroninski, Vladislav},
  journal={SIAM Journal on Mathematical Analysis},
  volume={45},
  number={5},
  pages={3019--3033},
  year={2013},
  publisher={SIAM}
}


@inproceedings{tarokh23,
  title={On conditions for uniqueness in sparse phase retrieval},
  author={Ohlsson, Henrik and Eldar, Yonina C},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2014 IEEE International Conference on},
  pages={1841--1845},
  year={2014},
  organization={IEEE}
}

@article{tarokh,
  title={New conditions for sparse phase retrieval},
  author={Ak{\c{c}}akaya, Mehmet and Tarokh, Vahid},
  journal={arXiv preprint arXiv:1310.1351},
  year={2013}
}



@article{survey2,
  title={Phase retrieval with application to optical imaging: a contemporary overview},
  author={Shechtman, Yoav and Eldar, Yonina C and Cohen, Oren and Chapman, Henry Nicholas and Miao, Jianwei and Segev, Mordechai},
  journal={Signal Processing Magazine, IEEE},
  volume={32},
  number={3},
  pages={87--109},
  year={2015},
  publisher={IEEE}
}

@article{survey1,
  title={Phase Retrieval: An Overview of Recent Developments},
  author={Jaganathan, Kishore and Eldar, Yonina C and Hassibi, Babak},
  journal={arXiv preprint arXiv:1510.07713},
  year={2015}
}


@inproceedings{phasecode,
  title={PhaseCode: Fast and efficient compressive phase retrieval based on sparse-graph codes},
  author={Pedarsani, Ramtin and Lee, Kangwook and Ramchandran, Kannan},
  booktitle={Communication, Control, and Computing (Allerton), 2014 52nd Annual Allerton Conference on},
  pages={842--849},
  year={2014},
  organization={IEEE}
}
@inproceedings{convexalgos,
  title={Sparse phase retrieval: Convex algorithms and limitations},
  author={Jaganathan, Kishore and Oymak, Samet and Hassibi, Babak},
  booktitle={Information Theory Proceedings (ISIT), 2013 IEEE International Symposium on},
  pages={1022--1026},
  year={2013},
  organization={IEEE}
}

@article{forgot38,
  author    = {Emmanuel J. Cand{\`{e}}s and
               Yonina C. Eldar and
               Thomas Strohmer and
               Vladislav Voroninski},
  title     = {Phase Retrieval via Matrix Completion},
  journal   = {CoRR},
  volume    = {abs/1109.0573},
  year      = {2011},
  url       = {http://arxiv.org/abs/1109.0573},
  timestamp = {Mon, 05 Dec 2011 18:05:29 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/abs-1109-0573},
  bibsource = {dblp computer science bibliography, http://dblp.org},
}

@article{shechtman2011sparsity,
  title={Sparsity based sub-wavelength imaging with partially incoherent light via quadratic compressed sensing},
  author={Shechtman, Yoav and Eldar, Yonina C and Szameit, Alexander and Segev, Mordechai},
  journal={Optics express},
  volume={19},
  number={16},
  pages={14807--14822},
  year={2011},
  publisher={Optical Society of America}
}



@article{forgot39,
  title={Phaselift: Exact and stable signal recovery from magnitude measurements via convex programming},
  author={Candes, Emmanuel J and Strohmer, Thomas and Voroninski, Vladislav},
  journal={Communications on Pure and Applied Mathematics},
  volume={66},
  number={8},
  pages={1241--1274},
  year={2013},
  publisher={Wiley Online Library}
}


@inproceedings{indyk,
 author = {Indyk, Piotr and Ngo, Hung Q. and Rudra, Atri},
 title = {Efficiently Decodable Non-adaptive Group Testing},
 booktitle = {Proceedings of the Twenty-first Annual ACM-SIAM Symposium on Discrete Algorithms},
 series = {SODA '10},
 year = {2010},
 isbn = {978-0-898716-98-6},
 location = {Austin, Texas},
 pages = {1126--1142},
 numpages = {17},
 url = {http://dl.acm.org/citation.cfm?id=1873601.1873692},
 acmid = {1873692},
 publisher = {Society for Industrial and Applied Mathematics},
 address = {Philadelphia, PA, USA},
} 


@article{rashad1990random,
  title={Random coding bounds on the rate for list-decoding superimposed codes},
  author={Rashad, AM},
  journal={PROBLEMS OF CONTROL AND INFORMATION THEORY-PROBLEMY UPRAVLENIYA I TEORII INFORMATSII},
  volume={19},
  number={2},
  pages={141--149},
  year={1990},
  publisher={PERGAMON-ELSEVIER SCIENCE LTD THE BOULEVARD, LANGFORD LANE, KIDLINGTON, OXFORD, ENGLAND OX5 1GB}
}

@book{du1999combinatorial,
  title={Combinatorial group testing and its applications},
  author={Du, Ding-Zhu and Hwang, Frank K},
  volume={12},
  year={1999},
  publisher={World Scientific}
}

@article{cdi1,
  title={Atomic resolution imaging of a carbon nanotube from diffraction intensities},
  author={Zuo, JM and Vartanyants, I and Gao, M and Zhang, R and Nagahara, LA},
  journal={Science},
  volume={300},
  number={5624},
  pages={1419--1421},
  year={2003},
  publisher={American Association for the Advancement of Science}
}

@article{cdi2,
  title={Coherent x-ray diffraction from quantum dots},
  author={Vartanyants, IA and Robinson, IK and Onken, JD and Pfeifer, MA and Williams, GJ and Pfeiffer, F and Metzger, H and Zhong, Z and Bauer, G},
  journal={Physical Review B},
  volume={71},
  number={24},
  pages={245302},
  year={2005},
  publisher={APS}
}

@article{cdi3,
  title={Three-dimensional mapping of a deformation field inside a nanocrystal},
  author={Pfeifer, Mark A and Williams, Garth J and Vartanyants, Ivan A and Harder, Ross and Robinson, Ian K},
  journal={Nature},
  volume={442},
  number={7098},
  pages={63--66},
  year={2006},
  publisher={Nature Publishing Group}
}

@article{cdi4,
  title={Coherent X-ray diffractive imaging: applications and limitations},
  author={Marchesini, S and Chapman, H and Hau-Riege, S and London, R and Szoke, A and He, H and Howells, M and Padmore, H and Rosen, R and Spence, J and others},
  journal={Optics Express},
  volume={11},
  number={19},
  pages={2344--2353},
  year={2003},
  publisher={Optical Society of America}
}




}


@article{de2005optimal,
  title={Optimal two-stage algorithms for group testing problems},
  author={De Bonis, Annalisa and Gasieniec, Leszek and Vaccaro, Ugo},
  journal={SIAM Journal on Computing},
  volume={34},
  number={5},
  pages={1253--1270},
  year={2005},
  publisher={SIAM}
}


@article{nature1,
  title={A compact X-ray free-electron laser emitting in the sub-angstrom region},
  author={Tanaka, Hitoshi and Yabashi, Makina and others},
  journal={Nat. Photonics},
  volume={6},
  pages={540--544},
  year={2012}
}

@article{nature2,
  title={First lasing and operation of an {\aa}ngstrom-wavelength free-electron laser},
  author={Emma, Paul and Akre, R and Arthur, J and Bionta, R and Bostedt, C and Bozek, J and Brachmann, A and Bucksbaum, P and Coffee, Ryan and Decker, F-J and others},
  journal={nature photonics},
  volume={4},
  number={9},
  pages={641--647},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{xray18,
  title={Lensless diffractive imaging using tabletop coherent high-harmonic soft-x-ray beams},
  author={Sandberg, Richard L and Paul, Ariel and Raymondson, Daisy A and H{\"a}drich, Steffen and Gaudiosi, David M and Holtsnider, Jim and Ra’anan, I Tobey and Cohen, Oren and Murnane, Margaret M and Kapteyn, Henry C and others},
  journal={Physical review letters},
  volume={99},
  number={9},
  pages={098103},
  year={2007},
  publisher={APS}
}

@article{xray19,
  title={Multiple wavelength diffractive imaging},
  author={Chen, Bo and Dilanian, Ruben A and Teichmann, Sven and Abbey, Brian and Peele, Andrew G and Williams, Garth J and Hannaford, Peter and Van Dao, Lap and Quiney, Harry M and Nugent, Keith A},
  journal={Physical Review A},
  volume={79},
  number={2},
  pages={023809},
  year={2009},
  publisher={APS}
}

@article{xray20,
  title={Ultrahigh 22 nm resolution coherent diffractive imaging using a desktop 13 nm high harmonic source},
  author={Seaberg, Matthew D and Adams, Daniel E and Townsend, Ethan L and Raymondson, Daisy A and Schlotter, William F and Liu, Yanwei and Menoni, Carmen S and Rong, Lu and Chen, Chien-Chun and Miao, Jianwei and others},
  journal={Optics express},
  volume={19},
  number={23},
  pages={22470--22479},
  year={2011},
  publisher={Optical Society of America}
}

@article{xray21,
  title={High numerical aperture tabletop soft x-ray diffraction microscopy with 70-nm resolution},
  author={Sandberg, Richard L and Song, Changyong and Wachulak, Przemyslaw W and Raymondson, Daisy A and Paul, Ariel and Amirbekian, Bagrat and Lee, Edwin and Sakdinawat, Anne E and Chan, La-O and Marconi, Mario C and others},
  journal={Proceedings of the National Academy of Sciences},
  volume={105},
  number={1},
  pages={24--27},
  year={2008},
  publisher={National Acad Sciences}
}

@article{xray22,
  title={Non-invasive imaging through opaque scattering layers},
  author={Bertolotti, Jacopo and van Putten, Elbert G and Blum, Christian and Lagendijk, Ad and Vos, Willem L and Mosk, Allard P},
  journal={Nature},
  volume={491},
  number={7423},
  pages={232--234},
  year={2012},
  publisher={Nature Publishing Group}
}


@inproceedings{bromberg,
  title={Efficient compressive phase retrieval with constrained sensing vectors},
  author={Bahmani, Sohail and Romberg, Justin},
  booktitle={Advances in Neural Information Processing Systems},
  pages={523--531},
  year={2015}
}

@article{berinde2008sparse,
  title={Sparse recovery using sparse random matrices},
  author={Berinde, Radu and Indyk, Piotr},
  journal={preprint},
  year={2008}
}

@article{baraniuk2014exponential,
  title={Exponential decay of reconstruction error from binary measurements of sparse signals},
  author={Baraniuk, Richard and Foucart, Simon and Needell, Deanna and Plan, Yaniv and Wootters, Mary},
  journal={arXiv preprint arXiv:1407.8246},
  year={2014}
}

@inproceedings{sigmadelta1,
  title={Sigma delta quantization for compressed sensing},
  author={G{\"u}nt{\"u}rk, C Sinan and Lammers, Mark and Powell, Alex and Saab, Rayan and Yilmaz, {\"O}zg{\"u}r},
  booktitle={Information Sciences and Systems (CISS), 2010 44th Annual Conference on},
  pages={1--6},
  year={2010},
  organization={IEEE}
}


@article{sigmadelta2,
  title={Sigma--Delta quantization of sub-Gaussian frame expansions and its application to compressed sensing},
  author={Krahmer, Felix and Saab, Rayan and Yilmaz, {\"O}zg{\"u}r},
  journal={Information and Inference},
  pages={iat007},
  year={2014},
  publisher={Oxford University Press}
}


@article{fastforeach,
  title={Approximate sparse recovery: optimizing time and measurements},
  author={Gilbert, Anna C and Li, Yi and Porat, Ely and Strauss, Martin J},
  journal={SIAM Journal on Computing},
  volume={41},
  number={2},
  pages={436--453},
  year={2012},
  publisher={SIAM}
}

@incollection{foreachlowrisk,
  title={l2/l2-foreach sparse recovery with low risk},
  author={Gilbert, Anna C and Ngo, Hung Q and Porat, Ely and Rudra, Atri and Strauss, Martin J},
  booktitle={Automata, Languages, and Programming},
  pages={461--472},
  year={2013},
  publisher={Springer}
}

@inproceedings{porat2012sublinear	,
  title={Sublinear time, measurement-optimal, sparse recovery for all},
  author={Porat, Ely and Strauss, Martin J},
  booktitle={Proceedings of the twenty-third annual ACM-SIAM symposium on Discrete Algorithms},
  pages={1215--1227},
  year={2012},
  organization={SIAM}
}


@article{goyal1998quantized,
  title={Quantized overcomplete expansions in IR N: analysis, synthesis, and algorithms},
  author={Goyal, Vivek K and Vetterli, Martin and Thao, Nguyen T},
  journal={Information Theory, IEEE Transactions on},
  volume={44},
  number={1},
  pages={16--31},
  year={1998},
  publisher={IEEE}
}

@inproceedings{jaganathan6,
  title={Recovery of sparse 1-D signals from the magnitudes of their Fourier transform},
  author={Jaganathan, Kishore and Oymak, Samet and Hassibi, Babak},
  booktitle={Information Theory Proceedings (ISIT), 2012 IEEE International Symposium On},
  pages={1473--1477},
  year={2012},
  organization={IEEE}
}

@inproceedings{jaganathan8,
  title={Phase retrieval for sparse signals using rank minimization},
  author={Jaganathan, Kishore and Oymak, Samet and Hassibi, Babak},
  booktitle={Acoustics, Speech and Signal Processing (ICASSP), 2012 IEEE International Conference on},
  pages={3449--3452},
  year={2012},
  organization={IEEE}
}

@article{jaganathan5,
  title={GESPAR: Efficient phase retrieval of sparse signals},
  author={Shechtman, Yoav and Beck, Andre and Eldar, Yonina C},
  journal={Signal Processing, IEEE Transactions on},
  volume={62},
  number={4},
  pages={928--938},
  year={2014},
  publisher={IEEE}
}

@article{jaganathan10,
  title={Simultaneously structured models with application to sparse and low-rank matrices},
  author={Oymak, Samet and Jalali, Amin and Fazel, Maryam and Eldar, Yonina C and Hassibi, Babak},
  journal={Information Theory, IEEE Transactions on},
  volume={61},
  number={5},
  pages={2886--2908},
  year={2015},
  publisher={IEEE}
}
@inproceedings{charikar2002finding,
  title={Finding frequent items in data streams},
  author={Charikar, Moses and Chen, Kevin and Farach-Colton, Martin},
  booktitle={International Colloquium on Automata, Languages, and Programming},
  pages={693--703},
  year={2002},
  organization={Springer}
}

